LLE with low-dimensional neighborhood representation

The local linear embedding algorithm (LLE) is a non-linear dimension-reducing technique, widely used due to its computational simplicity and intuitive approach. LLE first linearly reconstructs each input point from its nearest neighbors and then preserves these neighborhood relations in the low-dimensional embedding. We show that the reconstruction weights computed by LLE capture the high-dimensional structure of the neighborhoods, and not the low-dimensional manifold structure. Consequently, the weight vectors are highly sensitive to noise. Moreover, this causes LLE to converge to a linear projection of the input, as opposed to its non-linear embedding goal. To overcome both of these problems, we propose to compute the weight vectors using a low-dimensional neighborhood representation. We prove theoretically that this straightforward and computationally simple modification of LLE reduces LLE's sensitivity to noise. This modification also removes the need for regularization when the number of neighbors is larger than the dimension of the input. We present numerical examples demonstrating both the perturbation and linear projection problems, and the improved outputs using the low-dimensional neighborhood representation.

==> conclusions.tex <==
\section{Concluding remarks}\label{sec:conclusions}
to be written...
%
%We have argued that LLE in its existing form can fail to perform
%non-linear dimension reduction. We showed that the neighborhood
%description captures the structure of the high-dimensional space
%instead of the structure of the low-dimensional domain. We showed
%that this can cause As a result the algorithm converges to a linear
%projection of the high-dimensional input. We suggested a simple
%algorithm to overcome this problem that used local PCA to compute
%the reconstruction weight vectors. We showed some theoretical
%results and numerical examples for this algorithm. While this
%modification solves the problem of linear projection,

